A Lossless Deamortization for Dynamic Greedy Set Cover

The dynamic set cover problem has been subject to growing research attention in recent years. In this problem, we are given as input a dynamic universe of at most $n$ elements and a fixed collection of $m$ sets, where each element appears in a most $f$ sets and the cost of each set is in $[1/C, 1]$, and the goal is to efficiently maintain an approximate minimum set cover under element updates. Two algorithms that dynamize the classic greedy algorithm are known, providing $O(\log n)$ and $((1+\epsilon)\ln n)$-approximation with amortized update times $O(f \log n)$ and $O(\frac{f \log n}{\epsilon^5})$, respectively [GKKP (STOC'17); SU (STOC'23)]. The question of whether one can get approximation $O(\log n)$ (or even worse) with low worst-case update time has remained open -- only the naive $O(f \cdot n)$ time bound is known, even for unweighted instances. In this work we devise the first amortized greedy algorithm that is amenable to an efficient deamortization, and also develop a lossless deamortization approach suitable for the set cover problem, the combination of which yields a $((1+\epsilon)\ln n)$-approximation algorithm with a worst-case update time of $O(\frac{f\log n}{\epsilon^2})$. Our worst-case time bound -- the first to break the naive $O(f \cdot n)$ bound -- matches the previous best amortized bound, and actually improves its $\epsilon$-dependence. Further, to demonstrate the applicability of our deamortization approach, we employ it, in conjunction with the primal-dual amortized algorithm of [BHN (FOCS'19)], to obtain a $((1+\epsilon)f)$-approximation algorithm with a worst-case update time of $O(\frac{f\log n}{\epsilon^2})$, improving over the previous best bound of $O(\frac{f \cdot \log^2(Cn)}{\epsilon^3})$ [BHNW (SODA'21)]. Finally, as direct implications of our results for set cover, we [...]

==> DS.tex <==
\color{blue}
\section{Dominating Set}


\subsection{Overview}


\paragraph{Meeting Objective $1$ (Global Dirt).~}
It seems that our initial binary definition of active/passive must be ``level-sensitive" for it to work. Meaning, a vertex will be considered active \emph{up to a certain level}, and then passive \emph{from that level upwards}. Let us define the \emph{passive level} of a vertex $u \in V$ to be this certain level, denoted by $\plev(u)$, and roughly speaking it will be one level higher than the reset level of the highest reset in which $u$ participated in since there was last a deletion or insertion of an edge adjacent to $u$. A vertex $u$ will be ``clean" below its passive level, and ``dirty" at or above it, and it is important to have  $\lev(u) \le \plev(u)$ (see the discussion below). Denote by $A_k$ (respectively, $P_k$) the set of all vertices $u$ with $\lev(u) \le k$ and  $\plev(u)$ larger than (resp., no larger than) $k$. A vertex in $A_k$ (resp., $P_k$) will be called $k$-active (resp., $k$-passive). We define the system to be {\em $k$-dirty} if $|P_k| > 2\epsilon \cdot |A_k|$. Since $A_k \cup P_k$ is the set of all vertices dominated at level at most $k$, the system is $k$-dirty if roughly more than a $2\epsilon$-fraction of all vertices at level up to $k$ have a passive level also up to $k$.

\paragraph{Meeting Objective $2$ (Global Algorithm).~} 
We want to maintain the following invariant:

\begin{invariant}[see \Cref{invds} for more details]\label{ourds}
The following three conditions should hold:
	\begin{enumerate}[(1)]
 \item For any vertex $v$ in the current dominating set $D$, we have $\frac{|\dom(v)|}{\cost(v)}\geq \beta^{\lev_{\dom}(v)}$.
		\item Define $N_k(v) = A_k \cap N_+(v)$. For any vertex $v \in V$ and level $k$, we have $\frac{|N_k(v)|}{\cost(v)} < \beta^{k+1}$.	
  \item For any level $k$, we have $|P_k|\leq 2\epsilon \cdot|A_k|$.
	\end{enumerate}	
\end{invariant}

\noindent The first two conditions of the invariant correspond to the two in \Cref{global}, respectively. It may seem as though the first and second conditions imply local constraints, since they hold for each  vertex $v$. However, we make two crucial changes in the definitions: In the first condition, $\dom(v)$ is redefined to include also vertices $u$ that were dominated by $v$ but do to the deletion of $(u,v)$ they left $\dom(v)$, and $v$ has not yet gone through a reset. In such a case we will say that $u$ is a \emph{dead} vertex in $\dom(v)$ just to be consistent with the terminology in SC, even though following the edge update obviously $u$ is still alive but just dominated by some other vertex. In the second condition, $N_k(v)$ is redefined to consider only \emph{$k$-active} vertices. In a sense, these two conditions only consider ``clean" vertices. Lastly, we need to ensure that the vast majority of vertices are indeed ``clean". Meaning, we want to prevent the accumulation of too many $k$-passive vertices, for each $k$, otherwise the first two conditions would be meaningless, since a large fraction of vertices in the system would not be considered, which may blow up the approximation factor. To summarize, the first two conditions are local constraints that disregard all ``passive" vertices (for each level), and the third condition ensures that such passive vertices (for each level) are scarce, {\em and this is where the global relaxation for the first two comes into play}. Intuitively, the purpose of the third condition is to \emph{divert} dirt from the first two ``local" conditions (which are analogous to \Cref{global}) to the third, which is \emph{global} by design and thus crucial to achieve a fully global algorithm. 






To maintain this invariant we will execute a \emph{reset} up to level $k$ once $|P_k| > 2\epsilon \cdot|A_k|$, which amounts to running the static greedy algorithm on the subsystem of vertices that are dominated at a level up to $k$, and their neighbors. We want to trigger resets only once there is a violation to the third condition. 

When an edge $(u,v)$ is inserted, then it could be that (without loss of generality) $\lev_{\dom}(v) > \lev(u)$. In such a case, instead of \emph{transferring} $u$ from its previous $\dom(w)$ to $\dom(v)$, we \emph{copy} $u$ to $\dom(v)$, and now have another instantiation of $u$ in our solution. One \emph{alive} dominated by $v$, such that $\lev(u) = \plev(u) = \lev_{\dom}(v)$, and one \emph{dead} ``dominated" by $w$ (not actually dominated by $w$, but still in its dom set), such that $\lev(u) = \plev(u) = \lev_{\dom}(w)$. %In such a case we do not want to transfer $u$ from its previous $\dom(w)$ to $\dom(v)$, but rather leave $u$ in $\dom(w)$, and lower $\plev(u)$ to be $\lev(u)$. 
Notice that now $\plev(u)$ for the alive instantiation is no longer necessarily monotonically non-decreasing, but we maintain the fact that $\plev(u) \geq \lev(u)$. Notice that an insertion cannot reduce the size of $\dom(w)$ for any $w \in V$, since we can only mark a vertex as dead in $\dom(w)$ and copy it to a different dom set, and not transfer or remove it. Regarding $|N_k(w)|$, upon insertion of $(u,v)$, we lower $\plev(u)$ and $\plev(v)$ to be $\lev(u)$ and $\lev(v)$, respectively, for the old and new instantiations. If the passive level of a vertex is equal to its actual level, then by definition it cannot be in any $A_k$. Thus, insertion does not raise the size of $|N_k(w)|$, and we conclude that insertions cannot cause violations to the first two conditions, and instead they add ``passiveness" to the system, which will eventually trigger a violation to the third condition.  

When an edge $(u,v)$ is deleted, if say $u \in \dom(v)$, then we first mark $u$ in $\dom(v)$ as dead, then \emph{copy} $u$ to $\dom(w)$ such that $w \in N_+(u)$ that maximizes $\lev_{\dom}(w)$. If for all $w \in N_+(u)$ we have $\lev_{\dom}(w) = -1$ then create $\dom(u)$ such that $\dom(u) = \{u\}$. We set $\plev(u) = \lev(u) = \lev_{\dom}(w)$ in the alive instantiation, and set $\plev(u) = \lev(u) = \lev_{\dom}(v)$ in the dead one. Thus, here too, we now have another instantiation of $u$ in our solution. One \emph{alive} dominated by $w$, such that $\lev(u) = \plev(u) = \lev_{\dom}(w)$, and one \emph{dead} ``dominated" by $v$ (not actually dominated by $v$, but still in its dom set), such that $\lev(u) = \plev(u) = \lev_{\dom}(v)$. Similarly to insertions, here too deletions cannot cause violations to the first two conditions, and instead they add ``passiveness" to the system, which will eventually trigger a violation to the third condition.  



%we lower $\plev(u)$ and $\plev(v)$ to be $\lev(u)$ and $\lev(v)$, respectively. If the passive level of a vertex is equal to its actual level, then by definition it cannot be in any $A_k$. Thus, insertion does not raise the size of $|N_k(w)|$, and we conclude that insertions cannot cause violations to the first two conditions, and instead they add ``passiveness" to the system, which will eventually trigger a violation to the third condition.




%then $u$ joins $\dom(v)$ and leaves its previous $\dom(w)$. We then mark $u$ in $\dom(w)$ as dead. Now $\lev(u)$ will be $\lev_{\dom}(v)$, and $\plev(u)$ will be $\lev_{\dom}(w)$, since we want $v$ to be passive for level $\lev_{\dom}(w)$. Thus, it could be that $\plev(u) < \lev(u)$. 




%we will assign the passive level of each of its endpoints to be its actual level; 
%causing it to not be in any set $A_k$, and thus not in any $N_k(s)$, for any level $k$. In a sense, if the level and passive level of an element are equal, 
%in a sense, it can be considered as ``completely passive", 
%since if $\lev(e)=\plev(e)=j$, then $e \in P_{j'}$ for any $j' \geq j$. Therefore, insertions cannot raise
%since it cannot be in any set $A_k$ and $N_k(v)$ for any $k$ and $v$. 
%When an edge $(u,v)$ is deleted, if say $u \in \dom(v)$, then we first mark $u$ in $\dom(v)$ as dead, then assign $u$ to $\dom(w)$ where $w \in N_+(u)$ that maximized $\lev_{\dom}(w)$. If for all $w \in N_+(u)$ we have $\lev_{\dom}(w) = -1$ then create $\dom(u)$ such that $\dom(u) = \{u\}$.





%and assign its passive level to be its actual level. 

%Therefore, deletions cannot reduce the size of $\cov(s)$ for any $s$. Thus, insertions and deletions cannot cause violations to the first two conditions, and instead they add ``passiveness" to the system,
%by updating passive levels of elements, 
%which will eventually trigger a violation to the third condition. 

We want a reset up to level $k$ to completely ``clean up" everything up to $k$. Meaning, we would want $P_{k'}=\emptyset$ for any $k' \leq k$ following the reset. Thus, by definition of $P_k$, each participating vertex must have a passive level higher than $k$ following the reset. Not only do we want a reset to level $k$ to clean up everything up to that level, we also require that it would not create more dirt (or ``passiveness") in any higher level, otherwise a reset can trigger another (higher) reset, which could blow up the update time. We want only insertions and deletions to create dirt. Thus, if for example a reset to level $k$ is being executed and as a result a participating vertex $v$ wants to be created at level $k+5$, because it contains about $\cost(v) \cdot \beta^{k+5}$ participating vertices, we will not allow this, since this affects all levels between $k$ and $k+5$. Therefore, we will \emph{truncate} any reset to level $k$ at level $k+1$, meaning we will not allow participating vertices to dominate at any level higher than $k+1$. This way levels higher than $k$ are not affected by the reset, meaning there is no change to $P_{k'}$ and $A_{k'}$ for any $k' > k$, and notice that all participating vertices in a reset up to level $k$ will end up at a level up to $k+1$ following the reset. We conclude that following a reset to level $k$ the first two conditions still hold by design of the greedy algorithm and the level assignment in it, the third condition holds since $|P_{k'}|=0$ for any $k' \leq k$, and the reset has not raised $|P_{k'}|$ or lowered $|A_{k'}|$ for any $k' > k$, so this reset cannot trigger a reset at any higher level.

Since each participating vertex must have a passive level higher than $k$ following a reset to level $k$, each participating vertex will be assigned a passive level of the maximum between $k+1$ and its previous passive level. In this way, notice that the passive level of an element will never be lower than its level, and that the passive level of any vertex \textbf{between any two adjacent edge updates} is {\em monotonically non-decreasing}. This means that the number of different passive levels a vertex can go through during the update sequence is bounded by the number of levels in the system times the number of adjacent edge updates, and it turns out that this bound is what mandates the amortized update time to be $O(\Delta \cdot \log n)$, neglecting  dependencies on $\eps$ and $C$. 


To show this, consider a token scheme which gives each endpoint of the updated edge $O(\Delta)$ tokens for each passive level it could be at. The key observation is that even if there are multiple resets to the same  level $k$ throughout the update sequence, each vertex can only once be part of the collection $P_k$ that triggers the reset to level $k$ once $|P_k| > 2\epsilon \cdot|A_k|$, between any two adjacent edge updates, as afterwards its passive level would be at least $k+1$, and it will not decrease until the next adjacent edge update. Thus, we can give each vertex tokens to be responsible for only one reset for each level. Since a reset to level $k$ occurs once $|P_k|$ is (roughly) a $2\epsilon$-fraction of all vertices up to level $k$, handing out $O(\frac{\Delta}{\epsilon})$ tokens for each vertex per level would be enough to redistribute the tokens such that each participating vertex has $O(\Delta)$ tokens, enough to enumerate the neighboring vertices and update the corresponding data structures regarding the new level. We have thus obtained an algorithm with $O(\Delta \cdot \log n)$ amortized update time, 
%\footnote{The exact amortized update time is $O(\frac{\Delta \cdot \log (Cn)}{\epsilon^2})$, since there are roughly $\frac{\log (Cn)}{\epsilon}$ levels. In \Cref{sec:deam} we explain how to get rid of the $C$ factor.}, 
which maintains \Cref{ourds} that is based on our definition of global dirt. The final objective is to show that we achieve the desired approximation factor.





















\subsection{Preliminaries}


\begin{theorem}\label{warmupds}
	For any graph $G=(V,E)$, along with a cost function $\cost: V\rightarrow [1/C, 1]$, that undergoes a sequence of edge insertions and deletions, where the max-degree is always bounded by $\Delta$, and for any $\epsilon \in (0, \frac{1}{4})$, there is a dynamic algorithm that maintains a $((1+\epsilon)\ln n)$-approximate minimum dominating set in $O\brac{\frac{\Delta \log(Cn)}{\epsilon^2}}$ deterministic worst-case update time.
\end{theorem}


Although our claims are given in SC terminology for the sake of brevity, they can easily and readily be adapted to the DS problem. Following certain claims where the transition to DS might not be as trivial, we will add a remark regarding the adjustments necessary for the DS problem. In dynamic DS, edges are inserted or deleted, and we maintain a feasible set of vertices $D \subseteq V$ called a \emph{dominating set} such that the union of the sets of neighbors of each vertex in $D$ including the vertices in $D$ is equal to $V$. We denote by $\Delta$ the maximum degree of the dynamic graph throughout the update sequence (the analog of $f$). Each vertex $v$ has a cost (or weight), denoted $c(v)$, where $\frac{1}{C} \leq c(v) \leq 1$ for any $v \in V$. Denote by $N_+(v)$ the (dynamic) collection of vertices adjacent to some $v \in V$ including $v$. In the DS problem, each vertex has two roles: one as a dominating vertex and another as a dominated vertex. All vertices $v \in \mathcal{V}$ will be assigned a \emph{dominating} level value $\lev_{\dom}(v)\in [-1, L]$). We will assign each vertex $u \in V$ to one of the vertices $v \in D$, which we will denote by $\asn(u)$, and conversely, for each vertex $v \in V$, define its {\em dominating set} $\dom(v)$ to be the collection of vertices in $N_+(v)$ that are assigned to $v$, namely $\dom(v) = \{u\mid \asn(u) = v\}$. The \emph{dominated} level of a vertex $u$, denoted by $\lev(u)$ is defined as the dominating level of the vertex it is assigned to, namely $\lev(u) = \lev_{\dom}(\asn(u))$, and we make sure that $\lev(u) = \max\{\lev_{\dom}(v) \vert N_+(u) \ni v\}$, meaning $u$ is assigned to the vertex with the highest dominating level in $N_+(u)$. We define the dominating level of each vertex $v \notin D$ to be $-1$, whereas the dominating level of each vertex $v \in D$ will lie in $[0,L]$, so in particular we will have $\lev(u) \in [0, L]$, for each vertex $u \in V$. Let $D_i = \{v \mid \lev_{\dom}(v) = i \}, \forall i\in [-1, L]$, and $V_i = \{u \in V \mid \lev(u) = i\}, \forall i\in [0, L]$. Besides the dominated level value $\lev(v)$ for vertices $v$, we will also maintain a value of \emph{passive dominated level} $\plev(v)$ such that $\lev(v) \leq \plev(v) \leq L$, which plays a major role in our algorithm. In contrast to the dominated level $\lev(v)$ of a vertex $v$, which may decrease (as well as increase) by the algorithm, its passive dominated level $\plev(v)$ will be monotonically non-decreasing throughout its  lifespan.


\begin{definition} \label{multi}
We define the multiset $V^+ \supseteq V$ to be the multiset containing all instantiations of each vertex $u \in V$. Meaning, if some vertex $u \in V$ is in three dom sets, $\dom(v_1)$, $\dom(v_2)$ and $\dom(v_3)$ (where it is alive only in one), then $u$ will be in $V^+$ three times.
\end{definition}



\begin{definition} \label{actpassds}
For each level $k$, a vertex $v\in V$
is called \EMPH{$k$-active} (respectively, \EMPH{$k$-passive}) if 
$\lev(v) \leq k< \plev(v)$
(resp., $\plev(v)\leq k$)
and let $A_k = \{v\in V \mid \lev(v) \leq k< \plev(v)\}$ and $P_k = \{v\in V \mid \plev(v)\leq k\}$
be the sets of all $k$-active and $k$-passive vertices, respectively.
Notice that $A_k \cup P_k$ is the collection of all vertices dominated at level $\leq k$, and $A_k \cap P_k = \emptyset$. Moreover, if $A_k \cap P_{j} \neq \emptyset$ for two levels $k \ne j$, then $k < j$. For each vertex $v\in V$, define $N_k(v) = A_k\cap N_+(v)$.
\end{definition}

\begin{invariant} {\ } \label{invds}
	\begin{enumerate}[(1),leftmargin=*]
		\item For any vertex $v\in V$ and for each $k \in [0, L]$, we have $\frac{|N_k(v)|}{\cost(v)} < \beta^{k+1}$.
		\item For any vertex $v\in D$, we have $\frac{|\dom(v)|}{\cost(v)}\geq \beta^{\lev_{\dom}(v)}$;
  we note that $\dom(v)$ may include dead vertices.
  %, i.e., elements in $\univ^+ \setminus \univ$.
  In particular, $\lev_{\dom}(v)\leq \ceil{\log_\beta(Cn)}$.
		Moreover, for each $v \notin D$, $\lev_{\dom}(v) = -1$.
		\item For each $k \in [0, L]$, we have $|P_k|\leq 2\epsilon \cdot|A_k|$. We note that our algorithm does not maintain the values of $|P_k|, |A_k|$.
	\end{enumerate}
\end{invariant}





\begin{lemma}\label{toy-approx-ds}
	Let $D^*$ be an optimal dominating set for $V$. If \Cref{invds} is satisfied, then it holds that $\cost(D)\leq (1+O(\eps
	))\cdot \ln (\Delta + 1)\cdot \cost(D^*)$.
\end{lemma}




\begin{proof}
	By \Cref{invds}(3), we have for all $k \in [0,L-1]$:
	\begin{equation} \label{eq:inv313ds}
	\brac{\beta^{-k} - \beta^{-k-1}}\cdot |P_k| ~\leq~ 2\epsilon\cdot \brac{\beta^{-k} - \beta^{-k-1}}\cdot|A_k|.
	\end{equation}
	Taking a summation over all  $k\in \left[0, L-1\right]$, the left-hand side of \Cref{eq:inv313ds} becomes:
	$$\begin{aligned}
		\sum_{k = 0}^{L-1}(\beta^{-k} - \beta^{-k-1})\cdot |P_k| 
		&= \sum_{u\in V^+}\sum_{k = 0}^{L-1}(\beta^{-k} - \beta^{-k-1}) \cdot \ind[u\in P_k]\\
		&=\sum_{u\in V^+}\sum_{k = \plev(u)}^{L-1}(\beta^{-k} - \beta^{-k-1})\\
		& = \sum_{u\in V^+}\brac{\beta^{-\plev(u)}-\beta^{-L}}
	\end{aligned}$$
	and the right-hand side of \Cref{eq:inv313ds} becomes:
	$$\begin{aligned}
		2\epsilon\sum_{k = 0}^{L-1}(\beta^{-k} - \beta^{-k-1})\cdot |A_k| 
		&= 2\epsilon\sum_{u\in V^+}\sum_{k = 0}^{L-1}(\beta^{-k} - \beta^{-k-1}) \cdot \ind[u\in A_k]\\
		&= 2\epsilon\sum_{u\in V^+}\sum_{k = \lev(u)}^{\plev(u)-1}(\beta^{-k} - \beta^{-k-1})\\
		& = 2\epsilon\sum_{u\in V^+}\brac{\beta^{-\lev(u)}-\beta^{-\plev(u)}},
	\end{aligned}$$
	which yields:	
	$$\sum_{u\in V^+}\brac{\beta^{-\plev(u)}-\beta^{-L}}\leq 2\epsilon\cdot \sum_{u\in V^+}\brac{\beta^{-\lev(u)} - \beta^{-\plev(u)}}$$
	or equivalently, by adding $\sum_{u\in V^+}\brac{\beta^{-\lev(u)} - \beta^{-\plev(u)}}$ on the both sides, 
	\begin{equation} \label{eq:basicubds}
	\sum_{u\in V^+}\brac{\beta^{-\lev(u)}-\beta^{-L}} ~\leq~ (1+2\epsilon)\cdot \sum_{u\in V^+}\brac{\beta^{-\lev(u)} - \beta^{-\plev(u)}}.
	\end{equation}
	%We emphasize the point that $\univ^+$ also includes dead elements.

	%\shay{should clarify that $\univ$ here also counts dead elements}
	
	Next, let us lower bound $\cost(D^*)$ using the term $\sum_{u\in V^+}\brac{\beta^{-\lev(u)} - \beta^{-\plev(u)}}$. For any $v\in D^*$, consider the following three cases for any index $k\in [L]$: 
	\begin{itemize}
	\item $k < \log_\beta(1/\cost(v))-1$.
		
		By \Cref{invds}(1), we have: $|N_k(v)| < \beta^{k+1}\cdot \cost(v) < 1$, so $|N_k(v)| = 0$.
		
	
		\item $\log_\beta (1/\cost(v))-1\leq k \leq \log_\beta ((\Delta + 1)/\cost(v))$.
		
		By \Cref{invds}(1), we have: %\shay{should be $\beta^{-k-2}|N_k(s)|$, also in the third case}
		
		$$\frac{1}{\epsilon}\brac{\beta^{-k} - \beta^{-k-1}}|N_k(v)| = \beta^{-k-1}|N_k(v)| < \cost(v).$$
		
		
		\item $k > \ceil{\log_\beta ((\Delta + 1) / \cost(v))} = k_0$.
		
		In this case, we use the trivial bound: $|N_k(v)| \leq \Delta + 1 \leq \beta^{k_0}\cdot \cost(v)$, and so we have:
		$$\frac{1}{\epsilon}\brac{\beta^{-k} - \beta^{-k-1}}|N_k(v)| = \beta^{-k-1}|N_k(v)| \le \beta^{k_0 - k-1}\cdot \cost(v).$$
		
	%\shay{should be $\beta^{k_0 - k-2}$}
	\end{itemize}
%	Taking a summation over all $k\in [L]$, we can prove:
Observe that:
	\begin{equation} \label{lefthandds}
		\begin{aligned}
		\frac{1}{\epsilon} \sum_{k = 0}^{L-1}(\beta^{-k} - \beta^{-k-1})\cdot |N_k(v)| 
		&= \frac{1}{\epsilon}\sum_{u\in N_+(v)}\sum_{k = 0}^{L-1}(\beta^{-k} - \beta^{-k-1}) \cdot \ind[u\in N_k(v)]\\
		&= \frac{1}{\epsilon}\sum_{u\in N_+(v)}\sum_{k = \lev(u)}^{\plev(u)-1}(\beta^{-k} - \beta^{-k-1})\\
		& = \frac{1}{\epsilon}\sum_{u\in N_+(v)}\brac{\beta^{-\lev(u)}-\beta^{-\plev(u)}}.
	\end{aligned}
	\end{equation}
	By the above case analysis, we have:
	\begin{equation}
	\begin{aligned} \label{righthandds}
	\frac{1}{\epsilon} \sum_{k = 0}^{L-1}(\beta^{-k} - \beta^{-k-1})\cdot |N_k(v)|
	&= \frac{1}{\epsilon} \sum_{0 \le k < \log_\beta(1/\cost(v))-1}(\beta^{-k} - \beta^{-k-1})\cdot |N_k(v)| 
	\\&~~~+
	\frac{1}{\epsilon} \sum_{ \log_\beta(1/\cost(v))-1 \le k \le  \log_\beta ((\Delta + 1)/\cost(v))}(\beta^{-k} - \beta^{-k-1})\cdot |N_k(v)| 
	\\&~~~+
		\frac{1}{\epsilon} \sum_{\log_\beta ((\Delta + 1)/\cost(v)) < k \le L-1}(\beta^{-k} - \beta^{-k-1})\cdot |N_k(v)| 
	\\&<   \sum_{0 \le k < \log_\beta(1/\cost(v))-1} 0 
		\\&~~~+ 
  \sum_{ \log_\beta(1/\cost(v))-1 \le k \le  \log_\beta ((\Delta + 1)/\cost(v))} \cost(v) 
		\\&~~~+  \sum_{\log_\beta ((\Delta + 1)/\cost(v)) < k \le L-1}\beta^{k_0 - k - 1} \cost(v) 		
	\\&< \brac{0 + (\log_\beta(\Delta + 1) + 2) + 1/\epsilon}\cdot \cost(v).
	\end{aligned}
	\end{equation}
Combining \Cref{lefthandds} with \Cref{righthandds} yields
	$$\frac{1}{\epsilon}\sum_{u\in N_+(v)}\brac{\beta^{-\lev(u)}-\beta^{-\plev(u)}}\leq \brac{\log_\beta(\Delta + 1) + 2 + 1/\epsilon}\cdot \cost(v).$$
	Therefore, as $\ln(1+\epsilon) = \epsilon + O(\epsilon^2)$, under the assumption that $\eps =  \Omega(1 / \log (\Delta + 1))$ we have:
	$$\sum_{u\in N_+(v)}\brac{\beta^{-\lev(u)} - \beta^{-\plev(u)}}\leq
	(1+O(\epsilon))\ln (\Delta + 1)\cdot \cost(v).$$
	Since $D^*$ is a valid dominating set for all vertices in $V$, and as for each dead vertex instantiation of $u$ we have $\brac{\beta^{-\lev(u)} - \beta^{-\plev(u)}} = 0$ (because in any dead instantiation of $u$ we have $\lev(u) = \plev(u)$), 
 it follows that:
	
	%\shay{since $\univ$ might contain dead elements, should add another inequality for all alive elements but we don't have a notation for this} 
	%\shay{must assume that $\eps =  \Omega(1 / \log n)$}
	
	\begin{equation} \label{eq:concludeds} \sum_{u\in V^+}\brac{\beta^{-\lev(u)} - \beta^{-\plev(u)}} ~\leq~
	\sum_{v \in D^*} \sum_{u \in N_+(v)} (\beta^{-\lev(u)} - \beta^{-\plev(u)})
	~\le~ (1+O(\epsilon))\ln (\Delta + 1)\cdot \cost(D^*).
	\end{equation}
	
%	Finally, let us upper bound $\cost(\sets_\alg)$ with the term $\sum_{e\in \univ}\brac{\beta^{-\lev(e)} - \beta^{-L}}$. 
\noindent We conclude that
%\todo{I changed $\univ$ by $\univ^+$ in the following (and made other edits)}
%, we have the following inequality which finishes the proof:
$$\begin{aligned}
	\cost(D) &= \sum_{v\in D}\cost(v)\leq \sum_{v\in D}\beta^{-\lev_{\dom}(v)}\cdot |\dom(v)| ~=~ \beta\cdot \sum_{v\in D}\sum_{u\in \dom(v)}\beta^{-\lev(u)} 
	\\ &\le (1+O(\epsilon))\cdot \sum_{u\in V^+}\brac{\beta^{-\lev(u)} - \beta^{-L}}
	~\le~ (1+O(\epsilon))\cdot \sum_{u\in V^+}\brac{\beta^{-\lev(u)} - \beta^{-\plev(u)}}
	\\ &\le (1+O(\epsilon))\ln (\Delta + 1)\cdot \cost(D^*),
\end{aligned}$$
where the first inequality holds by \Cref{invds}(2), the second holds as $\lev(u)\leq L/2$ and hence $\beta^{-\lev(u)} - \beta^{-L} \ge \beta^{-\lev(u)}(1- \beta^{-\ceil{10\log_\beta 1/\epsilon}}) \ge \beta^{-\lev(u)}(1-\eps)$, and the last two follow from \Cref{eq:basicubds} and \Cref{eq:concludeds}, respectively.
% \shay{it should be $\beta^{\lev(s)}$ rather than $\beta^{1-\lev(s)}$}
\end{proof}
















\subsection{Algorithm Description} \label{sec:basAlgds}

We will skip the details for the fully global algorithm that maintains \Cref{invds}, with \emph{amortized} update time of $O(\frac{\Delta \cdot \log (Cn)}{\epsilon^2})$. Instead, we will dive straight into our ultimate goal of providing an algorithm that maintains \Cref{invds}, with a \emph{worst-case} update time of $O(\frac{\Delta \cdot \log (Cn)}{\epsilon^2})$ --- this is the result that underlies \Cref{warmupds}.
The main procedure of the algorithm is a {\em reset} operation, denoted by $\reset(k)$ when initiated for a level $k$. Simply put, performing a reset to level $k$ amounts to running the static greedy algorithm on the subgraph of vertices at level up to $k$.
Our algorithm distinguishes between procedures and data structures that are executed and maintained in the \emph{foreground} and those in the \emph{background}. The foreground procedures can be executed from start to finish between one adversarial update step to the next --- and as such are very basic procedures, and the foreground data structures support the foreground procedures and are used for explicitly maintaining the {\em output} solution at every update step.
In contrast, the background procedures can take a long time to run; the algorithm {\em simulates} their execution over a possibly long time interval in the background, and only upon termination of the execution, the main algorithm may ``copy'' the background data structures and their induced output
into the foreground data structures and their induced output.
In particular, the aforementioned reset operation will be running in the background, while adversarial insertions and deletions will be handled in a rather straightforward manner in the foreground. 
We note that for an amortized algorithm, there is no need for any background procedures, since everything can be executed on the foreground 
when needed. Meaning, once a reset needs to be executed, we just execute it in a single update step in the foreground. In this section we give a high level description of the algorithm, refer to \Cref{updtimeds} for more lower level details regarding the exact data structures maintained etc. 

\subsubsection{Foreground}

The dominating set solution $D$, which serves as the interface to the adversary (i.e., the output), will be maintained in the foreground. For the alive instantiation of any vertex $u \in V$, we maintain the following invariant:

\begin{invariant} \label{domdom}
$\lev(u) \geq \lev_{\dom}(u)$   
\end{invariant}


\noindent Edge deletions and insertions will be handled in the foreground as follows.

\begin{itemize}[leftmargin=*]
	\item \textbf{Deletions in the Foreground.} When an edge $(u,v)$ is deleted, if say (without loss of generality) $u \in \dom(v)$, then we first mark $u$ in $\dom(v)$ as dead, then \emph{copy} $u$ to $\dom(w)$ such that $w \in N_+(u)$ that maximizes $\lev_{\dom}(w)$. If for all $w \in N_+(u)$ we have $\lev_{\dom}(w) = -1$ then create $\dom(u)$ such that $\dom(u) = \{u\}$. We set $\plev(u) = \lev(u) = \lev_{\dom}(w)$ in the alive instantiation, and set $\plev(u) = \lev(u) = \lev_{\dom}(v)$ in the dead one. Thus, we now have another instantiation of $u$ in our solution. If neither vertex was in the other's dominating set prior to the deletion, then we just lower the passive level of the alive instances of each endpoint to be equal to the respective levels. Finally, for each $k \in [0,L]$ we feed the deletion of $(u,v)$ to instance $\reset(k)$ (if operating). 
 %Note that there is no need to feed the deletion of $e$ to instances of $\reset(k)$ with $k \leq \lev(e) - 1$, since $\reset(k)$ is not affected by (and does not affect) levels larger than $k+1$. See \Cref{delds} for the pseudo-code. 












 







 
\begin{algorithm} 
	\caption{$\textsf{Foreground-Delete}((u,v))$}\label{delds}
\If {alive $v \in \dom(u)$ \textbf{or} alive $u \in \dom(v)$ (WLoG alive $u \in \dom(v)$, cannot be both)}{
            mark $u$ as dead in $\dom(v)$\;
            $\lev(u), \plev(u) \leftarrow \lev_{\dom}(v)$ for the dead instantiation in $\dom(v)$\;
		$w=\arg\max_{w' \in N_+(u)}\{\lev_{\dom}(w')\}$\;
            $\lev(u), \plev(u) \leftarrow \lev_{\dom}(w)$ for the alive instantiation in $\dom(w)$\;
	}\Else{
		$\plev(u) \leftarrow \lev(u)$ for the alive instantiation\;   
	}
        $\plev(v) \leftarrow \lev(v)$ for the alive instantiation\;
	\For{$k$ from $0$ to $L$}{
		\If{$\reset(k)$ is operating}{
		feed this insertion to background system working on $\reset(k)$\;
		}
	}
\end{algorithm}	




 
	
\item \textbf{Insertions in the Foreground.} When an edge $(u,v)$ is inserted, then it could be that (without loss of generality) $\lev_{\dom}(v) > \lev(u)$. In such a case, instead of \emph{transferring} $u$ from its previous $\dom(w)$ to $\dom(v)$, we \emph{copy} $u$ to $\dom(v)$, and now have another instantiation of $u$ in our solution. One \emph{alive} dominated by $v$, such that $\lev(u) = \plev(u) = \lev_{\dom}(v)$, and one \emph{dead} ``dominated" by $w$ (not actually dominated by $w$, but still in its dom set), such that $\lev(u) = \plev(u) = \lev_{\dom}(w)$. 
Otherwise, we just lower the passive level of the alive instances of each endpoint to be equal to the respective levels. 
Finally, for each $k \in [0,L]$ we feed the deletion of $(u,v)$ to instance $\reset(k)$ (if operating). See \Cref{insds} for the pseudo-code.

\begin{algorithm}
	\caption{$\textsf{Foreground-Insert }((u,v))$} \label{insds} 
	\If {$\lev _{\dom }(u) > \lev (v)$ \textbf{or} $\lev _{\dom }(v) > \lev (u)$ (WLoG $\lev _{\dom }(v) > \lev (u)$, cannot be both)}{
		$\dom(v) \leftarrow \dom(v) \cup \{u\}$\;
            $\lev(u), \plev(u) \leftarrow \lev_{\dom}(v)$ for the alive instantiation in $\dom(v)$\;
		mark $u$ as dead in its previous $\dom(w)$\;
            $\lev(u), \plev(u) \leftarrow \lev_{\dom}(w)$ for the dead instantiation in $\dom(w)$\;
	}\Else{
		$\plev(u) \leftarrow \lev(u)$ for the alive instantiation\;   
	}
        $\plev(v) \leftarrow \lev(v)$ for the alive instantiation\;
	\For{$k$ from $0$ to $L$}{
		\If{$\reset(k)$ is operating}{
		feed this insertion to background system working on $\reset(k)$\;
		}
	}
\end{algorithm}	












































	
\item \textbf{Termination of $\reset(\cdot)$ Instances.} Upon any edge update (deletion or insertion), go over all levels $0\leq k\leq O(\log_\beta(Cn))$ and check if any instance $\reset(k)$ has just terminated right after the update. If so, take the largest such index $k$, and {\em switch its memory} to the foreground; we will describe how a memory switch is done later on in \Cref{termsecds}. After that, abort all instances of $\reset(i)$, for $0\leq i<k$.


\item \textbf{Initiating $\reset(\cdot)$ Instances.} Upon any edge update (deletion or insertion), go over all levels $0\leq k\leq L$ and check if there is currently an instance $\reset(k)$. Denote by $k_1,k_2,k_3, \ldots$ the levels that do not have such an instance, where $k_1 < k_2 < k_3 < \ldots$. Next, we want to partition all levels $k_i$ into \emph{short levels} and \emph{non-short levels}. All of the short levels will be lower than the non-short levels, meaning exists $i$ such that $k_{i'}$ is a short level for any $i'<i$ and a non-short level for any $i' \geq i$. In a nutshell, we will be able to execute a short level reset in a single update step, since the number of vertices participating in the reset is small enough. Recall that upon termination of a reset we abort all instances of lower level resets, thus there is no reason to run all short level resets, only the highest one. Regarding the non-short levels, we initiate a reset to each and every one of them. To find the highest short level given $k_1,k_2,k_3, \ldots$ we do as follows. First, count all the first $\frac{L}{\Delta}$ vertices, from dominated level $0$ upwards. Say that the $\frac{\Delta}{f}$-th element is at level $j$. Thus, we know that $|\bigcup_{i=0}^{j'} V_i| < \frac{\Delta}{f}$ for any $0 \leq j'<j$. Define $i$ to be the highest such that $k_i < j$. If no such $i$ exists then there are no short levels, otherwise $k_i$ is the highest short level, and we initiate the resets for levels $k_i,k_{i+1}, \ldots$, where again $k_i$ is a short level and the rest are non-short levels.

\end{itemize}




\subsubsection{Background}

For each level   $k\in [0, L]$, any reset instance $\reset(k)$ that operates (in the background) maintains a partial copy of the foreground in the background. Specifically, we maintain and define the following:
	\begin{enumerate}[(1),leftmargin=*]
		\item We maintain subsets of vertices $W^{(k)}, W^{(k)+}\subseteq V^+$
		($W^{(k)}$ are the alive vertex instantiations in $W^{(k)+}$), and for each vertex instance $w \in W^{(k)+}$, maintain the two level indices $\lev^{(k)}(w)$ and $\plev^{(k)}(w)$. In addition, we maintain a subset of vertices $B^{(k)} \subseteq V$, and a level value $\lev_{\dom}^{(k)}(b)$ for each $b\in B^{(k)}$, as well as a partial dominating set solution $D^{(k)}$ that dominates all vertices in $W^{(k)}$.
		
		\item For each level $i\in [-1, k+1]$, let $D_i^{(k)} = \{v \mid \lev_{\dom}^{(k)}(v) = i \}$ and for each level $i\in [0, k+1]$, let $V_i^{(k)} = \{u \mid \lev^{(k)}(u) = i\}$.
		
		\item For each vertex $w \in W^{(k)}$, we maintain the assignment $\asn^{(k)}(w)\in D^{(k)}$, and for each vertex $v \in D$ maintain the set $\dom^{(k)}(v)$, where $\dom^{(k)}(v) = \{w \mid \asn^{(k)}(w) = v\}$.
        \end{enumerate}





\begin{definition}\label{plands}
	The procedure $\reset(k)$ could make two different types of steps, \EMPH{immediate} and \EMPH{planned}: An immediate step of the algorithm is executed right away,
whereas a  planned step of the algorithm is stored implicitly in the background, and only executed when scheduled by the main algorithm in the foreground in reaction to edge updates. 
\end{definition}


\noindent As mentioned, for each level $k$, if there is currently no instance $\reset(k)$, then we start an instance $\reset(k)$ in the background if $k$ is either a non-short level or it is the highest short level. Then, after each adversarial update step, go over all non-short levels $k\in [0, L]$, and execute $O\brac{\Delta/\epsilon}$ \emph{planned} steps (see \Cref{plands}) of each instance of $\reset(k)$ (if operating), and execute the full reset of the short level reset. Roughly speaking, during the execution of an instance of $\reset(k)$, if an edge is inserted or deleted 
%on some level in the range $[0, k]$, 
then the background procedure $\reset(k)$ should also handle it. When an instance of $\reset(k)$ terminates, it will update all information on levels $\leq k$, and partly on level $k+1$,
%, within $O(\log n)$ time, by switching pointers to memory locations,
and then abort all other instances of $\reset(i), i<k$. 
The main technical part of our algorithm is the procedure $\reset(k)$, which runs in the background. 
Next, we describe the reset procedure, which consists of three phases: (I) initialization, (II) greedy dominating set algorithm, and (III) termination.

% as well as all the counters $|P_{i}|, |A_{i}|, i\in [0,k]$,

\paragraph{Phase I: Initialization.} When an instance of $\reset(k)$ has been initiated by the foreground, it sets the following:

\begin{itemize}
    \item $D^{(k)} = D_{i}^{(k)}  \leftarrow \emptyset, \forall i\in [0, k+1]$. 
    %Meaning, the collection of sets that will be chosen to cover the elements up to level $k$ begins empty.
    \item $V_{i}^{(k)} \leftarrow \emptyset, \forall i\in [0, k+1]$ 
    %Elements at each level up to $k$ will be determined by the reset (static greedy algorithm), and begins empty for each level.
    \item $W^{(k)}  = W^{(k)+} \leftarrow (\bigcup_{i=0}^k V_i) \cap V$. Meaning, the vertices participating in the reset are the ones that their alive instantiation is up to level $k$ in the foreground.
    \item $B^{(k)}\leftarrow$ all vertices that are adjacent to a vertex in $W^{(k)}$, including the vertices themselves. Thus, in particular, $W^{(k)} \subseteq B^{(k)}$. 
    %Note that we cannot create $B^{(k)}$ directly from the sets $D_k, D_{k-1}, \cdots, D_{-1}$, as there might be several vertices that do not dominate, and we do not want these sets to participate in a reset, since it could blow up the update time. 
    \item $\lev^{(k)}(w)\leftarrow -1, \forall w\in W^{(k)}$
    \item $\plev^{(k)}(w)\leftarrow \max\{\plev(w), k+1 \}, \forall w\in W^{(k)}$. Intuitively, following a reset to $k$ we want all vertices participating in this reset ($W^{(k)}$) to be active up to at least $k+1$ (without decreasing).
    \item $\lev_{\dom}^{(k)}(b) \leftarrow -1, \forall b\in B^{(k)}$
\end{itemize}



\noindent While the dominated level $\lev^{(k)}(w)$ of vertices $w$, initialized as $-1$, will be assigned 
a value from $0$ to $k+1$
throughout the execution of $\reset(k)$, the passive level $\plev^{(k)}(w)$ is assigned a value during initialization and does not change throughout the execution of $\reset(k)$. We note that $\plev^{(k)}(w)$ is no smaller than the foreground passive level
$\plev(w)$ of any vertex $w$, which will guarantee that the passive level of a vertex does not drop due to a reset. Moreover, $\plev^{(k)}(w)$ is at least $k+1$, which will guarantee that none of the vertices that participate in $\reset(k)$ from the initialization may belong to $P_i$, for any level $i \le k$. In addition, there is no effect to any level $j > k+1$, meaning if a vertex $w$ was $j$-passive before the reset to $k$, it will still be after, and if it was $j$-active, it will still be after.
For each vertex $v \in B^{(k)}$, we store the set $b \cap W^{(k)}$ (in a linked list). The stated steps incur a high running time, and as such cannot be executed in the foreground as immediate steps before the next update step occurs (aiming for a low worst-case update time), hence they will be scheduled as planned steps in the background. If during the initialization there is an edge deletion that causes the alive instantiation of a vertex $w$ to drop from $>k$ to $\leq k$, then we assign $\lev^{(k)}(w) = -1$ and $\plev^{(k)}(w) \leftarrow k+1$ (and it will participate in the reset). If during the initialization there is an edge insertion that causes the alive instantiation of a vertex $w$ to rise from $\leq k$ to $>k$, then we simply remove it from $W^{(k)}$. 


\paragraph{Phase II: Greedy Dominating Set Algorithm.} The algorithm consists of $k+2$ rounds, iterating from level $i = k+1$ down to $i = 0$;
in what follows, by writing ``the $i$th round'' we refer to the round that corresponds to level $i$. 
During the process, the algorithm maintains a collection $U \subseteq W^{(k)}$, which is the collection of all alive vertices that have not been dominated yet by the gradually growing $D^{(k)}$, and for each vertex $v \in B^{(k)}\setminus D^{(k)}$, it maintains all elements in $v\cap U$ (in a linked list). 
At the beginning of the $i$th round, we make the assumption below, which will be proven in \Cref{assum}.
\begin{assumption}\label{i-round-ds}
	The following two conditions hold {\em at the beginning} of the $i$th round. Importantly, these conditions do not necessarily hold throughout the $i$th round.
	\begin{itemize}[leftmargin=*]
		\item All vertices in $U$ are alive; this holds for any round $i = k+1,\ldots, 0$.
		\item For any round $i = k,\ldots,0$, $|N_+(v) \cap U| / \cost(v) < \beta^{i+1}$; for $i = k+1$, there is no upper bound on $|N_+(v) \cap U| / \cost(v)$.
	\end{itemize}
\end{assumption}

\noindent During the $i$th round, the following steps will be scheduled as planned.

\begin{framed}
	\noindent \textbf{Planned Steps in the $i$th Round.}
	During the $i$th round, the algorithm iteratively chooses a vertex $v \in B^{(k)}\setminus D^{(k)}$ that maximizes $|N_+(v) \cap U| / \cost(v)$ such that $|N_+(v) \cap U| / \cost(v) \geq \beta^i$. This will be implemented by a \emph{truncated max-heap}. If no such $v$ exists and $i>0$, we proceed to the next ($i-1$) round.  
 %of top priority
	%from the truncated max-heap, with a lower bound threshold of $\beta^i$. 
	%As long as the top priority set $s$ satisfies $|s\cap U| / \cost(s) \geq \beta^i$, we perform the following steps. 
	Add $v$ to $D^{(k)}$, assign $\lev_{\dom}^{(k)}(v) \leftarrow i$, and then go over all alive vertices $u \in N_+(v)\cap U$ and assign $\lev^{(k)}(u)\leftarrow i, \asn^{(k)}(u)\leftarrow v$; note that $\plev^{(k)}(u)$ was already assigned for vertices that existed at the beginning of this phase, and, as described below, it is also assigned for vertices newly joined to $W^{(k)}$.  
After that, we remove $u$ from $U$ and enumerate all vertices $v^\prime$ such that $u \in N_+(v^{\prime})$ to maintain
%the linked list 
$v^\prime\cap U$. 
%[[S: should also update the key in the truncated heap]]

	%\tianyi{Doesn't this take $O(\log^2n)$ time in total per element? We should do something nontrivial to calculate the counters.}
\end{framed}


\noindent See \Cref{resetds} for the pseudo-code of the planned steps in the greedy dominating set algorithm. 


\begin{algorithm}
	\caption{Phase II of $\reset(k)$ - Greedy Dominating Set Algorithm} \label{resetds}
	\For{$i$ from $k+1$ to 0}{
		NoVertex $\leftarrow$ FALSE\;
		\While{(!NoVertex)}{
			choose a vertex $v \in B^{(k)}\setminus D^{(k)}$ that maximizes $|N_+(v) \cap U| / \cost(v)$\;
			\If{($|N_+(v) \cap U| / \cost(v) < \beta^i$) \textbf{\emph{or}} ($B^{(k)}\setminus D^{(k)} = \emptyset$)}{
				NoVertex $\leftarrow$ TRUE\;
			}
			\Else{
				$D^{(k)} \leftarrow D^{(k)} \cup \{v\}$\;
				$\lev_{\dom}^{(k)}(v) \leftarrow i$\;
				\For{$u \in N_+(v) \cap U$}{
					$\lev^{(k)}(u) \leftarrow i$\;
					$\asn^{(k)}(u) \leftarrow v$\;
					$U \leftarrow U \setminus \{u\}$\;
					\For{$v' \in N_+(u)$}{
						$N_+(v') \cap U \leftarrow N_+(v') \cap U \setminus \{u\}$\;
                            Update heap\;
					}
     }
				}
			}
		}
		%\For{$j$ from $i$ to $k$}{
		%	update $|P^{(k)}_j|$ and $|A^{(k)}_j|$\;
		%}
\end{algorithm}



\noindent Finally, we describe how to handle adversarial edge updates that are fed to the background during the $i$th round.

\begin{itemize}[leftmargin=*]

\item \textbf{Deletions in the Background.} 

Suppose that an edge $(u,v)$ is deleted by the adversary during the $i$th round. If either vertex is currently in $B^{(k)} \setminus D^{(k)}$, then first update the heap by enumerating $|N_+(v) \cap U|$ and $|N_+(u) \cap U|$. If no vertex dominated the other, we do not do anything else. If without loss of generality $v$ dominated $u$, and as a result $u$ joins some $\dom(w)$, we proceed as follows. Following the deletion, we have a dead instantiation of $u$ at level $\lev_{\dom}(v)$ and an alive instantiation of $u$ at level $\lev_{\dom}(w)$, where $\lev_{\dom}(v) \geq \lev_{\dom}(w)$. If $\lev_{\dom}(w) > k$, we do not need to do anything, since $\reset(k)$ does not need to take care of this vertex. If $\lev_{\dom}(v) \leq k$, then $u$ already participates in the reset. The only issue is if $\lev_{\dom}(v) > k$ and $\lev_{\dom}(w) \leq k$. Meaning, before the deletion $\lev(u) > k$ and after $\lev(u) \leq k$, both in the foreground. In such a case we want to ``insert" $u$ to the reset, similarly as done in the set cover problem. We enumerate all vertices $u' \in N_+(u)$, and proceed as follows:

\begin{itemize}[leftmargin=*]
 
\item If $u$ is adjacent to a vertex in $D^{(k)}$ (and thus dominated by $D^{(k)}$), then find such a vertex $u' \in D^{(k)}$ that maximizes $\lev_{\dom}^{(k)}(u')$, and then assign $\lev^{(k)}(u) = \plev^{(k)}(u)\leftarrow \lev_{\dom}^{(k)}(u')$. Note that such vertices will not have $\plev^{(k)} \ge k+1$ as vertices that participate from the beginning of the execution of $\reset(k)$.
	
\item Otherwise, $u$ is not dominated by $D^{(k)}$, in which case we assign $\plev^{(k)}(u)\leftarrow i, \lev^{(k)}(u)\leftarrow -1$. Such vertices might be dominated throughout this or subsequent rounds of $\reset(k)$, which will change their $\lev^{(k)}(u)$ to be the round in which they are dominated, i.e., at most $i$, but their $\plev^{(k)}(u)$ will remain $i$; note also the difference from vertices that participated from the beginning of the execution of $\reset(k)$.

\item Regardless of whether $u$ is dominated by a vertex in $D^{(k)}$ or not, we need to add all vertices not in $B^{(k)}$ in $N_+(u)$ to $B^{(k)} \setminus D^{(k)}$. There are at most $\Delta + 1$ such vertices, and for each such vertex $u'$ we know that $N_+(u') \cap U = \{u\}$, since otherwise $u'$ would have already been in $B^{(k)}$. Therefore, we can update the heap in $O(\Delta)$ time.

\end{itemize}

\item \textbf{Insertions in the Background.} 

Suppose that an edge $(u,v)$ is inserted by the adversary during the $i$th round. If either vertex is currently in $B^{(k)} \setminus D^{(k)}$, then first update the heap by enumerating $|N_+(v) \cap U|$ and $|N_+(u) \cap U|$. If due to the insertion, without loss of generality $u$ becomes dead in $\dom(w)$ and joins $\dom(v)$, where $\lev_{\dom}(w) \leq k$ and $\lev_{\dom}(v) > k$, then we want to ``delete" $u$ from the reset, similarly as done in the set cover problem. We mark $u$ as dead (thus it joins $W^{(k)+} \setminus W^{(k)}$), and assign $\plev^{(k)}(u)\leftarrow \lev^{(k)}(u)$. If $u$ is in $U$ at the moment, we remove $u$ from $U$, enumerate all vertices $u' \in N_+(u)$, update the linked list $N_+(u') \cap U$, and update the truncated max-heap.
	
\end{itemize}


\paragraph{Phase III: Termination.} When all $(k+2)$ rounds of the greedy dominating set algorithm terminate, we set $D_i$ and $V_i$ (foreground) to be $D_i^{(k)}$ and $S_i^{(k)}$, respectively, for each $i\in [0, k]$. Then, append the linked list of $D_{k+1}^{(k)}$ and $V_{k+1}^{(k)}$ to $D_{k+1}$ and $V_{k+1}$. Finally, we abort all lower-level reset instances. 

\subsection{Implementation Details and Update Time Analysis} \label{updtimeds}

The implementation and update time analysis for the dominating set problem is almost identical to that of the set cover problem described in \Cref{updtime}, with the obvious analogous terms ($\Delta+1$ instead of $f$, etc.). Thus, we omit the details to avoid unnecessary repetition. We conclude that any insertion/deletion in the foreground can be dealt with in $O(\Delta \cdot L)$ time, thus it can be done within a single update step. Dealing with the short level reset (finding the highest one, initializing the reset, and executing the greedy dominating set algorithm) takes $O(L)$ time, thus it will all be done within a single update step as well. Likewise, termination can be done in $O(L)$ time (updating data structures of the highest finished reset and aborting the rest). Every other $\reset(k)$ will take $O(\Delta \cdot |W^{(k)}|)$ time (initialization and greedy dominating set algorithm). Since this cannot be executed within a single update step, for each $k$ we will execute $O(\frac{\Delta}{\epsilon})$ computations per update step. In \Cref{proofcorrectds} we will prove that by working in such a pace, we can ensure that \Cref{invds} holds, which in turn will be enough to prove that the approximation factor holds, by \Cref{toy-approx-ds}.





\subsection{Proof of Correctness} \label{proofcorrectds}

The following two claims hold for the dominating set problem analogously to the set cover problem in \Cref{consistency} and \Cref{assum}, respectively.

\begin{claim}\label{consistencyds}
The foreground data structures $\{D_k\}_{-1\leq k\leq L}, \{V_k\}_{0\leq k\leq L}$ are consistent; that is, they satisfy their specifications in \Cref{warmupds}.
\end{claim}

\begin{claim} \label{assumds}
\Cref{i-round-ds} always holds.
\end{claim}

Next, we prove that \Cref{invds} always holds in the foreground, which concludes the proof of \Cref{warmupds}.






\begin{claim}\label{inv1ds}
	\Cref{invds}(1) always holds in the foreground.
\end{claim}

\begin{proof}

First, observe that an edge insertion/deletion cannot cause a violation to \Cref{invds}(1), it just adds ``passiveness" to the system (and hence can cause a violation to \Cref{invds}(3) only). Since insertions and deletions to the foreground cannot cause a violation to \Cref{inv}(1), the only possibility is if \Cref{invds}(1) is violated in the background in some system working on $\reset(k)$, and it is then transferred to the foreground. Assume by contradiction that exists a vertex $v$ such that upon termination of $\reset(k)$, we have $\frac{|N_j(v)|}{\cost(v)} \geq \beta^{j+1}$ for some $j$.

If $j \geq k+1$, then for $|N_j(v)|$ to grow between right before the initialization of $\reset(k)$ and right after the termination of $\reset(k)$, there must exist a vertex $u \in N_+(v)$ that joined $N_j(v)$ sometime between those two time steps. First, observe that the passive level of $u$ cannot grow from $\leq j$ to $>j$ due to the reset. Thus, the passive level of $u$ had to be higher than $j$ in the beginning of the reset, and its level must have been $>j$ and dropped to $\leq j$. This too cannot occur in an instance of $\reset(k)$ for $j \geq k+1$.

%For this to happen $u$ must change its passive level, since its level cannot fall from $>j$ to $\leq j$ in an instance of $\reset(k)$ where $j \geq k+1$ (because $u$ would not participate in such a reset). This means that when $\reset(k)$ is initialized, either $\plev(e) \leq j$ or $e$ has not been inserted yet, and $\plev(e) > j$ when $\reset(k)$ terminates. Consider the first case where $\plev(e) = i$ when the reset is initialized, where $i \leq j$. Then by the algorithm description $\plev(e)$ is $\max\{i,k+1\}$ when the reset terminates. But clearly $j \geq \max\{i,k+1\}$ and so we reach a contradiction. Now consider the second case where $e$ was inserted sometime during the execution of $\reset(k)$. By the algorithm description $\plev(e)$ is $\leq k+1$ when the reset terminates, and since $j \geq k+1$ we again reach a contradiction.

If $j < k+1$, we claim that all vertices in $N_j(v)$ at the termination of $\reset(k)$ were in $U$ in the beginning of round $j$. Assume by contradiction that exists a vertex $u \in N_j(v)$ when the reset terminates, such that $u \notin U$ in the beginning of round $j$. If $u$ was added to $U$ during round $j$ or after, then at termination $\plev(u) \leq j$ by the algorithm description (because $\lev(u) \leq j$ by definition of $N_j(v)$), a contradiction to the fact that $u \in N_j(v)$ when the reset terminates. If $u$ participated in the reset, but was not in $U$ in the beginning of round $j$, it means it has already been dominated in a previous round, meaning dominated at a level $>j$, which again is a contradiction to the fact that $u \in N_j(v)$ when the reset terminates. So indeed all vertices in $N_j(v)$ at the termination of $\reset(k)$ were in $U$ in the beginning of round $j$. But since we assumed by contradiction that upon termination $\frac{|N_j(v)|}{\cost(v)} \geq \beta^{j+1}$, we get that $\frac{|N_+(v) \cap U|}{\cost(v)} \geq \beta^{j+1}$ in the beginning of round $j$, a contradiction to \Cref{i-round-ds}. 
\end{proof}


\begin{claim}\label{inv2ds}
	\Cref{invds}(2) always holds in the foreground.
\end{claim}

\begin{proof}

It is immediate by the algorithm description that the second half of \Cref{invds}(2) (that $\lev_{\dom}(v) = -1$ for each $v \notin D$) always holds. It remains to show that $|\dom(v)| / \cost(v) \ge \beta^{\lev_{\dom}(v)}$, for any vertex $v \in D$. Since $\dom(v)$ can contain dead vertices as well, clearly an insertion/deletion cannot cause a violation to this invariant. Thus the only possibility left is if \Cref{invds}(2) is violated in the background in some system working on $\reset(k)$, and it is then transferred to the foreground. Assume by contradiction that exists a vertex $v$ such that upon termination of $\reset(k)$, we have $|\dom(v)| / \cost(v) < \beta^{\lev_{\dom}(v)}$. By the description of the greedy dominating set algorithm, when a vertex $v$ joins the partial solution $D^{(k)}$ during the $i$th round, it is guaranteed that $|\dom(v)| / \cost(v) = |N_+(v) \cap U| / \cost(v) \geq \beta^i = \beta^{\lev_{\dom}^{(k)}(v)}$; recalling that $\dom(v)$ also includes dead vertices, this ratio $|\dom(v)| / \cost(v)$ may only increase later on.
\end{proof}

\begin{claim} \label{pre4invds}
	Consider an instance of $\reset(k)$ and denote by $U_i$ the collection of undominated vertices at the beginning of round $i$ in the greedy dominating set algorithm phase, where $i\in [0, k+1]$. Then by working at a pace of $O(\Delta / \epsilon)$ per update step, the reset will terminate after less than $\frac{\epsilon}{4} |U_i|$ edge updates following the beginning of round $i$.
 \end{claim}

\begin{proof}
	Note that at the beginning of round $i$, the total number of remaining planned computations by $\reset(k)$ is $O(\Delta |U_i|)$, since each remaining vertex will change its level only once, and it will take $O(\Delta)$ time for it to update all relevant data structures regarding this change. Each time the adversary makes an update, the number of vertices joining the reset can be at most one, so if we mark by $x$ the total number of update steps from the beginning of round $i$ until termination, there are at most $|U_i| + x$ vertices that we need to assign to levels, taking $O(\Delta(|U_i|+x))$ time. Notice though that $x$ is roughly $\epsilon |U_i|$, since the reset takes care of $\Theta(\frac{1}{\epsilon})$ vertices per update step ($\Theta(\frac{\Delta}{\epsilon})$ computations per update step, each element taking $\Theta(\Delta)$ time), in which time only one can join. So $O(\Delta(|U_i|+x)) = O(\Delta|U_i|)$, meaning the reset takes $O(\Delta|U_i|)$ time for planned and immediate steps. By working at a pace of $O(\frac{\Delta}{\epsilon})$ computations per update step, we can finish all steps in less than $\frac{\epsilon}{4} |U_i|$ update steps. 
\end{proof}

\begin{claim} \label{claim4invds}
	Following the termination of an instance $\reset(k)$, we have $|P_i| < \epsilon \cdot |A_i|$ for all $i \leq k$.
\end{claim}

\begin{proof}
	Consider the moment when the $i$th round of the greedy dominating set algorithm begins in an instance of $\reset(k)$ (within Phase II of $\reset(k)$), where $i\in [0, k+1]$. Denote by $U_i$ the set of all currently undominated vertices.
	By \Cref{pre4invds}, the reset will terminate in less than $\frac{\epsilon}{2} |U_i|$ update steps. By the algorithm description,
	each vertex $u \in U_i$ 
	 at the beginning of the $i$th round will be assigned $\lev(u)$ at most $i$ in round $i$ onwards, while $\plev(u) > i$. The only vertices that could have level $\leq i$ with passive level also $\leq i$, and thus
	belong to $P^{(k)}_{i}$, are endpoints of inserted/deleted edges by the adversary from the $i$th round onwards. As mentioned, there are less than $\frac{\epsilon}{4} |U_i|$ insertions/deletions from this point until termination, so at the end of the reset $|P^{(k)}_{i}|<\frac{\epsilon}{2} |U_i|$. Moreover, $(|A^{(k)}_{i}| + |P^{(k)}_{i}|)$ at the end of the reset is the total number of vertices that were assigned to a level up to $i$. 
 %To give a lower bound to this, we know that there are less than $\frac{\epsilon}{2} |U_i|$ deletions from the $i$th round onwards [[S: I think that the deleted ``dead'' elements, are also counted in $P^{(k)}_{i}$, so I'm not sure we need to consider them separately]]. 
 So eventually there will be at least $|U_i|$
 %$ - \frac{\epsilon}{2} |U_i|$ 
 vertices (alive and dead) dominated at level $\leq i$, meaning $(|A^{(k)}_{i}|  + |P^{(k)}_{i}|) \geq |U_i|$
 %- \frac{\epsilon}{2} |U_i|$ [[S: my understanding is that	$(|A^{(k)}_{i}|  + |P^{(k)}_{i}|) \ge |U_i|$, since even the dead elements are counted here]]. 
 Combining this altogether we obtain that $|P^{(k)}_{i}| < \epsilon |A^{(k)}_{i}|$ for any $\epsilon < 0.5$. 
	%and only one such insertion is enough for there would be more than $|U|$ elements eventually at level $\leq i$, we get that $|A^{(k)}_{i}| \geq |U| \geq \frac{1}{\epsilon}|P^{(k)}_{i}|$.
\end{proof}

\begin{claim} \label{largerds}
	When $\reset(k)$ terminates and is transferred to the foreground, it does not change $A_{k'}$, and $P_{k'}$ can only reduce in size, for any $k'>k$.
\end{claim}

\begin{proof}

%First, we will show that each vertex in $P_{k'}$ in the foreground before the termination of $\reset(k)$ remains there after the termination. Consider such a vertex $u \in P_{k'}$. $\plev^{(k)}(u) \leq k'$ upon termination, since otherwise that would mean that $\plev(u) > k'$ following $\reset(k)$, and since this cannot happen due to the reset (the passive level would be at least $k+2$), we must have had $\plev(u) > k'$ in the foreground upon termination, a contradiction to the fact that $u \in P_{k'}$ in that time. The only exception is if $u$ was a dead vertex, therefore it was in $P_{k}$ thus in $P_{k'}$ as well, and $e$ would be completely removed during the reset, reducing $|P_{k'}|$ by one.

First, we will show that each vertex in $A_{k'}$ in the foreground before the termination of $\reset(k)$ remains there after the termination. Consider such a vertex $u \in A_{k'}$. Clearly $\lev^{(k)}(u) \leq k'$ upon termination, since $u$ cannot rise to a level above $k+1$, which is $\leq k'$. Since $u \in A_{k'}$, the passive level of $u$ in the foreground right before termination of $\reset(k)$ is $> k'$, thus it is also $> k+1$. Therefore, the passive level of $u$ would not have changed due to $\reset(k)$, and $u$ remains in $A_{k'}$.

Next, we will show that no new vertices join $A_{k'}$ following the termination of $\reset(k)$. Assume by contradiction that exists such a vertex $u$. Either $\lev(u) > k'$ or $\plev(u) \leq k'$ in the foreground right before the termination. If $\lev(u) > k'$, then the only way $u$ would have participated in $\reset(k)$, is if before the termination of $\reset(k)$ there was a termination of some $\reset(k'')$ where $k'' \geq k'$. This would abort $\reset(k)$ though. If $\plev(u) \leq k'$, then since $k' \geq k+1$, by the algorithm description $\plev^{(k)}(u)$ will remain $\leq k'$, a contradiction.

Finally, we will show that no new vertices join $P_{k'}$ following the termination of $\reset(k)$. Assume by contradiction that exists such a vertex $u$. Either $\lev(u) > k'$ or $\plev(u) > k'$ in the foreground right before the termination. If $\lev(u) > k'$, then the only way $u$ would have participated in $\reset(k)$, is if before the termination of $\reset(k)$ there was a termination of some $\reset(k'')$ where $k'' \geq k'$. This would abort $\reset(k)$ though. Likewise, if $\plev(u) > k'$ in the foreground right before the termination, then since the passive level cannot decrease, $u$ cannot join $P_{k'}$, and the claim follows.
%then before the termination of $\reset(k)$ there was a termination of some $\reset(k'')$ where $k'' \geq k'$, which again, would abort $\reset(k)$.
%$P_k$ doesn't become too large - first, no element that was previously in $A_k$ joins $P_k$, as they had plev at least $k+1$, and the active level will not exceed $k$, so they will remain in $A_k$. 
%	Next, what about newly inserted elements and elements of $A_{k-1} \cup P_{k-1}$ (I focus on the case $k'+1 = k$)? 
%	They may belong to $P_k$. As for the ``old elements'', we can argue that they must have already belonged to $P_k$ - if they move to $P_k$, then their passive level is at most $k$ also before the reset (if it were higher than $k$ previously, and as it won't decrease, they wouldn't move to $P_k$). As for the new elements; first, we can employ the previous claim to reason that only $\eps/2 \cdot |U_{k'}| \le \approx \eps \cdot |A_k|$ new elements may join $P_k$, but I think we can say something stronger: all these newly inserted elements that might increase $|P_{k}|$ in the background are anyway increasing $P_k$ in the foreground, so it seems that there is no special overhead due to the background treatment of new elements.
\end{proof}
%Since each element update can raise $|P^{(k)}_{i}|$ by only one, at the end of the reset procedure we have $|P^{(k)}_{i}|\leq \epsilon |U|$. On the other hand, b

%Next, we show that the third part of \Cref{inv} holds.

\noindent The following lemma is completely analogous to \Cref{inv3}, and can be proved in the same way using \Cref{pre4invds}, \Cref{claim4invds} and \Cref{largerds} (instead of \Cref{pre4inv}, \Cref{claim4inv} and \Cref{larger} respectively). 
\begin{lemma}\label{inv3ds}
	\Cref{invds}(3) always holds in the foreground.
\end{lemma}

\begin{comment}

\begin{proof}

Assume by contradiction that there exists $k$ such that $|P_k| > 2\epsilon \cdot |A_k|$ for some $k$, at the end of update step $t$ (right before update step $t+1$). Let $t'$ be the last time step before $t$ that $\reset(k)$ was initiated. $\reset(k)$ was initiated at time $t'$ right after the termination of some $\reset(k')$, where $k' \geq k$, by the algorithm description. By \Cref{claim4inv}, we know that at time $t'$ (following the termination of $\reset(k')$) we have $|P_k| < \epsilon \cdot |A_k|$ in the foreground.

Between $t'$ and $t$, $|P_k|$ can rise and $A_k$ can change only due to insertions/deletions, since by definition of $t'$ no termination of $\reset(k')$ for any $k' \geq k$ exists, and any termination of $\reset(k')$ for any $k' < k$ would not raise $|P_k|$ or change $A_k$ by \Cref{larger}. By denoting $A_k$ at times $t'$ and $t$ by $A_k^{t'}$ and $A_k^{t}$ respectively, we conclude that there must be more than ($2\epsilon \cdot |A_k^{t}| - \epsilon \cdot |A_k^{t'}|$) update steps between $t'$ and $t$, since again due to one insertion/deletion only one element can join $P_k$. 
	
%As mentioned, at update step $t'$, $\reset(k)$ is already working in the background. Say this reset was initiated at time step $t'' \leq t'$, and let $\tau = t'' - t'$ (so $\tau \geq 0$). 
If we denote by $x$ the total number of update steps throughout which $\reset(k)$ is executed, we get by Claim \ref{pre4inv} that:

	
	\begin{equation} \label{inv3eq1}
		x < \frac{\epsilon}{2}(|P_k^{t'}| + |A_k^{t'}|),
	\end{equation} 
	
	\noindent since the collection of all elements participating in $\reset(k)$ initiated at time $t'$ is $P_k^{t'} \cup A_k^{t'}$. We assume that at update step $t$, $\reset(k)$ is still running, thus we will reach a contradiction if:
	
	\begin{equation} \label{inv3eq2}
		\frac{\epsilon}{2}(|P_k^{t'}| + |A_k^{t'}|) < 2\epsilon \cdot |A_k^{t}| - \epsilon \cdot |A_k^{t'}|.
	\end{equation} 
	
	\noindent Now, notice that:
	
	\begin{equation} \label{inv3eq3}
		|A_k^{t}| \geq |A_k^{t'}| - x,
	\end{equation} 
	
	\noindent since again, in each update step during the reset up to one element can be removed from $A_k$, and we assumed that $x \geq t-t'$. Thus, we need to show that:
	
	\begin{equation} \label{inv3eq4}
		\frac{\epsilon}{2}(|P_k^{t'}| + |A_k^{t'}|) < 2\epsilon \cdot (|A_k^{t'}|-x) - \epsilon \cdot |A_k^{t'}|.
	\end{equation} 
	
	\noindent Plugging in $x$ from \Cref{inv3eq1} and rearranging, we get that we need to show:
	
	\begin{equation} \label{inv3eq5}
		(\frac{1}{2} + \epsilon)|P_k^{t'}| < (\frac{1}{2} - \epsilon)|A_k^{t'}|.
	\end{equation} 
	
	\noindent Since we know that $|P_k^{t'}| < \epsilon|A_k^{t'}|$, it is enough to show that:

        \begin{equation} \label{inv3eq5.5}
		(\frac{1}{2} + \epsilon) \cdot \epsilon|A_k^{t'}| < (\frac{1}{2} - \epsilon)|A_k^{t'}|,
	\end{equation} 

\noindent meaning that 

        \begin{equation} \label{inv3eq6}
		2\epsilon^2 + 3\epsilon -1 < 0,
	\end{equation} 

 \noindent which holds for any $\epsilon < \frac{1}{4}$.	
%	\noindent Rearranging, we get that this inequality holds for any $\epsilon < 0.1$ and $|A_k^{t'}| > \frac{5}{\epsilon}$. In the special case where $t'=t$, $\reset(k)$ will terminate within a single update step, at the end of time step $t'$, since a reset with $O(\frac{1}{\epsilon})$ participating elements is computed in $O(\frac{f}{\epsilon} + \log_{\beta}n)$ running time. 
Thus, we reach our contradiction and the lemma follows.

\end{proof}

\end{comment}



We conclude that our algorithm indeed maintains \Cref{invds}, in worst-case update time of $O(\frac{\Delta \cdot L}{\epsilon}) = O\brac{\frac{\Delta\log(Cn)}{\epsilon^2}}$ as described in \Cref{updtimeds}. Since \Cref{invds} holds, the approximation factor of the maintained minimum set cover is $(1+\epsilon)\ln (\Delta + 1)$, as shown in \Cref{toy-approx-ds}. This concludes the proof of \Cref{warmupds}.






\subsection{Removing Dependency on Aspect Ratio} \label{removecds}

To remove the dependency on $C$ in the update time, we employ the same black-box reduction from \Cref{remove} for the set cover problem. 
%\shay{I stop here; I'll first read Section 3 and then return to this point}
Define the \emph{top level} of vertex $v$ as $\tlev(v) = \ceil{\log_\beta(n / \cost(v))}$. Define a parameter $K = \ceil{10\log_\beta n}$.
\begin{definition}
	For any $l\geq -1$, define $V_l = \{v\in V\mid \tlev(v)\in [lK, (l+2)K) \}$, and let $U_l$ be the (dynamic) collection of all vertices such that the cheapest vertex adjacent to them (including them) is in $V_l$.
\end{definition}

\begin{remark}
Note that in the dominating set problem, vertices in $U_l$ can leave to $U_{l'}$ for some $l' \neq l$, whereas in the set cover problem the sets containing an element remained static throughout its lifetime. Upon each edge update though only one vertex can become dead in one $U_l$ and be added to another $U_{l'}$, so in a sense each edge update can be thought of as a vertex deletion from one system and an insertion to another.
\end{remark}

\noindent For each $l\geq -1$, we will maintain a dominating set $D_{l}\subseteq V_l$ that dominates $U_l$ by applying \Cref{warmupds} as a black-box which takes $O\brac{\frac{\Delta \log n}{\epsilon^2}}$ worst-case update time. Overall, by \Cref{ob1} and \Cref{ob2} we will have two different dominating set solutions for all vertices:
$$D_{\even} = \bigcup_{j\geq 0}D_{2j} \; , \; D_{\odd} = \bigcup_{j\geq 0}D_{2j-1}. $$
Following similar lines to those in the argument for the set cover problem, it can be proved that at least one solution from $\{D_{\even}, D_{\odd} \}$ is a $(1+\epsilon) \ln (\Delta + 1)$-approximation; we next provide this argument, for completeness, which would complete the proof of \Cref{wc2ds}.

\begin{lemma}\label{approxlow}
	For any $l\geq -1$, let $k_0\in I_l$ be the smallest index such that there exists a set in $\mathcal{S}_l$ covering at level $k_0$, or in other words, $k_0$ is the smallest level such that $\sets_{l, \alg}\cap S_{l, k_0}\neq \emptyset$. If $k_0 \leq (l+1)K$, then we have:
	$$\sum_{j \geq 0}\cost(\sets_{l + 2j, \alg})\leq (1+O(\epsilon))f \cdot \cost(\sets^*).$$
\end{lemma}
\begin{proof}
    We know that 
$\cost(\sets_{l, \alg}) \le (1+O(\epsilon))f \cdot \cost(\sets^*_l) \le (1+O(\epsilon))f \cdot \cost(\sets^*)$. 
%Next, let us prove that $\sum_{j\geq 1}\cost(\sets_{l+2j, \alg})\leq \epsilon\cdot \cost(\sets_{l,\alg})$. 
Consider any set $s_0\in \sets_{l, \alg}\cap S_{l, k_0}$. For any set $s\in \sets_{l+2j, \alg}$ and $j>0$, we have: 
	\begin{equation} \label{costs2} \cost(s)\leq n \cdot \beta^{1-\tlev(s)}\leq n\cdot \beta^{1-(l+2)K} \leq n\cdot \beta^{1-k_0-K} \leq \frac{\epsilon}{(1+2\epsilon) n}\cdot\beta^{-k_0-1}\leq \frac{\epsilon\cdot\cost(s_0)}{(1+2\epsilon) n},
 \end{equation}
	
\noindent where the first inequality holds since  $\tlev(s) \leq \log_\beta (n / \cost(s)) + 1$
(by definition of $\tlev(s)$), the second holds since $\tlev(s) \geq (l+2j)K \ge (l+2)K$ for any $j>0$ by definition of $s$, the third follows from the initial assumption that $k_0 \leq (l+1)K$, the fourth by definition of $K$ and that $\epsilon > \frac{2}{n^8}$ is not too small, and the fifth holds since $s_0$ is covering at level $k_0$. %Since each element is assigned to one set in the set cover, and only up to a $\frac{2\epsilon}{1+2\epsilon}$-fraction of the elements can be dead (otherwise \Cref{inv-scale}(3) is violated) 
Since at most $n$ elements are alive and at most $2\eps \cdot n$ elements may be dead (otherwise
\Cref{lastinv}(3) is violated), and as each element (dead or alive) is assigned to at most one set in the set cover solution, it follows that the total number of sets in
$\sets_{l+2j, \alg}$ over all $j>0$
is bounded by $(1+2\epsilon) n$. By \Cref{costs2}, we get $$\sum_{j>0}\cost(\sets_{l+2j, \alg}) ~\leq~
(1+2\eps)n \cdot \left(\frac{\epsilon}{(1+2\epsilon) n}\cdot\cost(s_0)\right)
~\le~
\epsilon\cdot\cost(s_0) ~\leq~ \epsilon\cdot \cost(\sets_{l, \alg}).$$ We conclude that
$$\sum_{j \geq 0}\cost(\sets_{l + 2j, \alg}) ~=~ \cost(\sets_{l, \alg}) + \sum_{j>0}\cost(\sets_{l+2j, \alg}) ~\leq~ (1+\epsilon) \cdot \cost(\sets_{l, \alg}) ~\leq~ (1+O(\epsilon))f \cdot \cost(\sets^*),$$
\noindent and the lemma follows.
\end{proof}

\noindent Next, by following the same lines of \Cref{approxf} (with $f$ instead of $\ln n$) and using \Cref{approxlow}, we can show that: $$\min\{\cost(\sets_{\even, \alg}), \cost(\sets_{\odd, \alg}) \}\leq (1+O(\epsilon))f \cdot \cost(\sets^*),$$

\noindent and we have thus concluded the proof of \Cref{wc2}.












\color{black}

==> figs/scale-free.tex <==
\begin{tikzpicture}[thick,scale=0.7]
	\draw (0, 13.2) node[inner sep=0pt, minimum width=6pt, label=\textbf{level}] {};
	
	\draw (-2, -1) node [circle, draw, fill=black, inner sep=0pt, minimum width=6pt, label=90: {$e\in\univ_l$}] {};
	\draw (-2, -2) node[inner sep=0pt, minimum width=6pt, label=$\lev_l(e)$] {};
	
	\draw (2, 1) node [circle, draw, fill=black, inner sep=0pt, minimum width=6pt, label=90: {$e\in\univ_{l+1}$}] {};
	\draw (2, 0) node[inner sep=0pt, minimum width=6pt, label=$\lev_{l+1}(e)$] {};

	\draw (-4.5, -2.4) node[label={$I_l$}]{};
	\draw (4.5, 0.8) node[label={$I_{l+1}$}]{};
	\draw (-4.5, 4.4) node[label={$I_{l+2}$}]{};
	\draw (4.5, 7.4) node[label={$I_{l+3}$}]{};

	\begin{scope}[on background layer]
		\draw [->, line width = 0.5mm] (0, -5) to (0, 13);
		
		\draw [line width = 1mm, color=red] (-2, -4) to (0, -4);
		\draw [line width = 1mm, color=red] (-2, -3) to (0, -3);
		\draw [line width = 1mm, color=red] (-2, -2) to (0, -2);
		
		\draw [line width = 1mm, color=red] (-2, -1) to (2, -1);
		\draw [line width = 1mm, color=red] (-2, 0) to (2, 0);
		\draw [line width = 1mm, color=red] (-2, 1) to (2, 1);
		
		\draw [line width = 1mm, color=red] (0, 2) to (2, 2);
		\draw [line width = 1mm, color=red] (0, 3) to (2, 3);
		\draw [line width = 1mm, color=red] (0, 4) to (2, 4);
						
		%\draw [line width = 0.2mm, style={decorate, decoration=snake}] (1) to (2);
		
		\draw [decorate, decoration={calligraphic brace,amplitude=5pt}, line width=1.5pt] (-3.5, -5) -- (-3.5, 1.5);
				
		\draw [decorate, decoration={calligraphic brace,amplitude=5pt}, line width=1.5pt] (3.5, 4.6) -- (3.5, -1.6);
		
		\draw [decorate, decoration={calligraphic brace,amplitude=5pt}, line width=1.5pt] (-3.5, 1.8) -- (-3.5, 8.3);
		
		\draw [decorate, decoration={calligraphic brace,amplitude=5pt}, line width=1.5pt] (3.5, 11.2) -- (3.5, 5);
	\end{scope}
\end{tikzpicture}

==> nuggets.tex <==


